HAT-P-68b: A Transiting Hot Jupiter Around a K5 Dwarf Star

We report the discovery by the ground-based HATNet survey of the transiting exoplanet HAT-P-68b, which has a mass of 0.724 $\pm$ 0.043 $M_{Jup}$, and radius of 1.072 $\pm$ 0.012 $R_{Jup}$. The planet is in a circular P = 2.2984-day orbit around a moderately bright V = 13.937 $\pm$ 0.030 magnitude K dwarf star of mass 0.673 $+$ 0.020 $-$0.014 $M_{\odot}$, and radius 0.6726 $\pm$ 0.0069 $R_{\odot}$. The planetary nature of this system is confirmed through follow-up transit photometry obtained with the FLWO~1.2m telescope, high-precision RVs measured using Keck-I/HIRES, FLWO~1.5m/TRES, and OHP~1.9m/Sophie, and high-spatial-resolution speckle imaging from WIYN~3.5m/DSSI. HAT-P-68 is at an ecliptic latitude of $+3^{\circ}$ and outside the field of view of both the NASA TESS primary mission and the K2 mission. The large transit depth of 0.036 mag ($r$-band) makes HAT-P-68b a promising target for atmospheric characterization via transmission spectroscopy.

==> HTR268-002.empirical.tex <==
\newcommand{\hatcurhtrempirical}{HTR268-002}                       % Original HTR name of target
\newcommand{\hatcurfieldempirical}{\ensuremath{string}}            % HTR field
\newcommand{\hatcurCCraempirical}{\ensuremath{07^{\mathrm h}53^{\mathrm m}55.97{\mathrm s}}}                     % Right Ascension
\newcommand{\hatcurCCdecempirical}{\ensuremath{+23{\arcdeg}56{\arcmin}17.6{\arcsec}}}                    % Declination
\newcommand{\hatcurCCmagempirical}{14.020}                         % apparent V-band magnitude
\newcommand{\hatcurCCtwomassempirical}{2MASS~07535598+2356176}     % 2MASS identifier
\newcommand{\hatcurCCgscempirical}{GSC~1925-01046}                 % GSC(1.2) identifier
\newcommand{\hatcurCCtassmvempirical}{\ensuremath{14.020\pm0.079}} % APASS V-band magnitude
\newcommand{\hatcurCCtassmvshortempirical}{\ensuremath{14.0}}      % APASS V-band magnitude
\newcommand{\hatcurCCtassmBempirical}{\ensuremath{15.32\pm0.17}}   % APASS B-band magnitude
\newcommand{\hatcurCCtassmBshortempirical}{\ensuremath{15.3}}      % APASS B-band magnitude
\newcommand{\hatcurCCtassmIempirical}{\ensuremath{nff\pmnff}}      % TASS I-band magnitude
\newcommand{\hatcurCCtassmIshortempirical}{\ensuremath{0.0}}       % TASS I-band magnitude
\newcommand{\hatcurCCtassmgempirical}{\ensuremath{14.71\pm0.13}}   % APASS g-band magnitude
\newcommand{\hatcurCCtassmgshortempirical}{\ensuremath{14.7}}      % APASS g-band magnitude
\newcommand{\hatcurCCtassmrempirical}{\ensuremath{13.485\pm0.076}} % APASS r-band magnitude
\newcommand{\hatcurCCtassmrshortempirical}{\ensuremath{13.5}}      % APASS r-band magnitude
\newcommand{\hatcurCCtassmiempirical}{\ensuremath{13.25\pm0.42}}   % APASS i-band magnitude
\newcommand{\hatcurCCtassmishortempirical}{\ensuremath{13.2}}      % APASS i-band magnitude
%% --------------------------------------------------------------------
\newcommand{\hatcurCCtwomassJmagempirical}{\ensuremath{11.750\pm0.022}} % 2MASS ORIG MAG
\newcommand{\hatcurCCtwomassHmagempirical}{\ensuremath{11.210\pm0.023}} % 2MASS ORIG MAG
\newcommand{\hatcurCCtwomassKmagempirical}{\ensuremath{11.019\pm0.018}} % 2MASS ORIG MAG
\newcommand{\hatcurCCcitJmagempirical}{\ensuremath{11.748\pm0.023}} % 2MASS CIT MAG
\newcommand{\hatcurCCcitHmagempirical}{\ensuremath{11.202\pm0.024}} % 2MASS CIT MAG
\newcommand{\hatcurCCcitKmagempirical}{\ensuremath{11.043\pm0.019}} % 2MASS CIT MAG
\newcommand{\hatcurCCbbJmagempirical}{\ensuremath{11.826\pm0.025}} % 2MASS BB MAG
\newcommand{\hatcurCCbbHmagempirical}{\ensuremath{11.226\pm0.025}} % 2MASS BB MAG
\newcommand{\hatcurCCbbKmagempirical}{\ensuremath{11.063\pm0.019}} % 2MASS BB MAG
\newcommand{\hatcurCCesoJmagempirical}{\ensuremath{11.833\pm0.029}} % 2MASS ESO MAG
\newcommand{\hatcurCCesoHmagempirical}{\ensuremath{11.225\pm0.036}} % 2MASS ESO MAG
\newcommand{\hatcurCCesoKmagempirical}{\ensuremath{11.060\pm0.020}} % 2MASS ESO MAG
\newcommand{\hatcurCCesoJHmagempirical}{\ensuremath{0.608\pm0.043}} % 2MASS ESO JH COLOR
\newcommand{\hatcurCCesoJKmagempirical}{\ensuremath{0.773\pm0.033}} % 2MASS ESO JK COLOR
\newcommand{\hatcurCCesoHKmagempirical}{\ensuremath{0.165\pm0.040}} % 2MASS ESO HK COLOR
%% --------------------------------------------------------------------
\newcommand{\hatcurLCdipempirical}{\ensuremath{3.6}}               % BLS detected dip (mmag)
\newcommand{\hatcurLCrprstarempirical}{\ensuremath{0.16114\pm0.00052}} % Rp/R*
\newcommand{\hatcurLCbsqempirical}{\ensuremath{0.0150_{-0.0067}^{+0.0071}}} % impact parameter square
\newcommand{\hatcurLCimpempirical}{\ensuremath{0.122_{-0.031}^{+0.026}}} % impact parameter
\newcommand{\hatcurLCzetaempirical}{\ensuremath{26.744\pm0.087}}   % zeta/R*
\newcommand{\hatcurLCdurempirical}{\ensuremath{0.08700\pm0.00031}} % transit duration (days)
\newcommand{\hatcurLCdurshortempirical}{\ensuremath{0.0870}}       % transit duration (days)
\newcommand{\hatcurLCdurhrempirical}{\ensuremath{2.0879\pm0.0074}} % transit duration (hours)
\newcommand{\hatcurLCdurhrshortempirical}{\ensuremath{2.088}}      % transit duration (hours)
\newcommand{\hatcurLCqempirical}{\ensuremath{0.03790\pm0.00015}}   % fractional transit duration (days)
\newcommand{\hatcurLCqshortempirical}{\ensuremath{0.038}}          % fractional transit duration (days)
\newcommand{\hatcurLCingdurempirical}{\ensuremath{0.012233\pm0.000095}} % ingress/egress duration (days)
\newcommand{\hatcurLCPempirical}{\ensuremath{2.29840696\pm0.00000029}} % period (days)
\newcommand{\hatcurLCPprecempirical}{\ensuremath{2.2984070}}       % period (days)
\newcommand{\hatcurLCPshortempirical}{\ensuremath{2.2984}}         % period (days)
\newcommand{\hatcurLCTempirical}{\ensuremath{2456919.891980\pm0.000063}} % epoch (BJD)
\newcommand{\hatcurLCTAempirical}{\ensuremath{2455876.41522\pm0.00019}} % TA (BJD)
\newcommand{\hatcurLCTBempirical}{\ensuremath{2457480.703275\pm0.000011}} % TB (BJD)
\newcommand{\hatcurLChatnetmempirical}{\ensuremath{13.44122\pm0.00021}} % HATNet OOT level
\newcommand{\hatcurLCiblendempirical}{\ensuremath{0.901\pm0.035}}  % HATNet iblend factor
%% --------------------------------------------------------------------
\newcommand{\hatcurSMEiteffempirical}{\ensuremath{4514\pm50}}      % Ini SME, stellar effective temperature
\newcommand{\hatcurSMEizfehempirical}{\ensuremath{-0.140\pm0.080}} % Ini SME, stellar metallicity
\newcommand{\hatcurSMEizfehshortempirical}{\ensuremath{-0.14}}     % Ini SME, stellar metallicity
\newcommand{\hatcurSMEiloggempirical}{\ensuremath{4.67\pm0.10}}    % Ini SME, stellar surface gravity
\newcommand{\hatcurSMEivsinempirical}{\ensuremath{0.0\pm2.0}}      % Ini SME, stellar rotational velocity
\newcommand{\hatcurSMEivmacempirical}{\ensuremath{0.0}}            % Ini SME, stellar macroturbulence
\newcommand{\hatcurSMEivmicempirical}{\ensuremath{0.0}}            % Ini SME, stellar microturbulence
%% --------------------------------------------------------------------
\newcommand{\hatcurLBizempirical}{\ensuremath{0.3598}}             % Limb darkening parameters, Gamma1, z-band
\newcommand{\hatcurLBiizempirical}{\ensuremath{0.2452}}            % Limb darkening parameters, Gamma2, z-band
\newcommand{\hatcurLBiiempirical}{\ensuremath{0.4552}}             % Limb darkening parameters, Gamma1, i-band
\newcommand{\hatcurLBiiiempirical}{\ensuremath{0.2183}}            % Limb darkening parameters, Gamma2, i-band
\newcommand{\hatcurLBiIempirical}{\ensuremath{0.4216}}             % Limb darkening parameters, Gamma1, I-band
\newcommand{\hatcurLBiiIempirical}{\ensuremath{0.2285}}            % Limb darkening parameters, Gamma2, I-band
\newcommand{\hatcurLBigempirical}{\ensuremath{0.8947}}             % Limb darkening parameters, Gamma1, g-band
\newcommand{\hatcurLBiigempirical}{\ensuremath{-0.0532}}           % Limb darkening parameters, Gamma2, g-band
\newcommand{\hatcurLBirempirical}{\ensuremath{0.6186}}             % Limb darkening parameters, Gamma1, r-band
\newcommand{\hatcurLBiirempirical}{\ensuremath{0.1455}}            % Limb darkening parameters, Gamma2, r-band
\newcommand{\hatcurLBiRempirical}{\ensuremath{0.5726}}             % Limb darkening parameters, Gamma1, R-band
\newcommand{\hatcurLBiiRempirical}{\ensuremath{0.1672}}            % Limb darkening parameters, Gamma2, R-band
\newcommand{\hatcurLBikepempirical}{\ensuremath{0.1000}}           % Limb darkening parameters, Gamma1, Kep-band
\newcommand{\hatcurLBiikepempirical}{\ensuremath{0.1000}}          % Limb darkening parameters, Gamma2, Kep-band
%% --------------------------------------------------------------------
\newcommand{\hatcurISOmempirical}{\ensuremath{0.684\pm0.015}}      % stellar mass
\newcommand{\hatcurISOmshortempirical}{\ensuremath{0.68}}          % stellar mass
\newcommand{\hatcurISOmlongempirical}{\ensuremath{0.684\pm0.015}}  % stellar mass
\newcommand{\hatcurISOrempirical}{\ensuremath{0.6786\pm0.0054}}    % stellar radius
\newcommand{\hatcurISOrshortempirical}{\ensuremath{0.68}}          % stellar radius
\newcommand{\hatcurISOrlongempirical}{\ensuremath{0.6786\pm0.0054}} % stellar radius
\newcommand{\hatcurISOrhoempirical}{\ensuremath{3.089\pm0.046}}    % stellar density (cgs)
\newcommand{\hatcurISOrholongempirical}{\ensuremath{3.089\pm0.046}} % stellar density (cgs)
\newcommand{\hatcurISOloggempirical}{\ensuremath{4.6100\pm0.0058}} % stellar surface gravity from isochrones
\newcommand{\hatcurISOlumempirical}{\ensuremath{0.1305\pm0.0053}}  % stellar luminosity
\newcommand{\hatcurISOlumshortempirical}{\ensuremath{0.13}}        % stellar luminosity
\newcommand{\hatcurISOmvempirical}{\ensuremath{7.369\pm0.094}}     % stellar absolute magnitude
\newcommand{\hatcurISOviempirical}{\ensuremath{100\pm0}}           % stellar V-I index
\newcommand{\hatcurISOageempirical}{\ensuremath{0\pm0}}            % stellar age
\newcommand{\hatcurISOteffempirical}{\ensuremath{4216\pm34}}       % stellar Teff
\newcommand{\hatcurISOMJempirical}{\ensuremath{5.581\pm0.026}}     % stellar absolute J magnitude
\newcommand{\hatcurISOMHempirical}{\ensuremath{4.816\pm0.037}}     % stellar absolute H magnitude
\newcommand{\hatcurISOMKempirical}{\ensuremath{4.687\pm0.032}}     % stellar absolute K magnitude
\newcommand{\hatcurISOJKempirical}{\ensuremath{0.890\pm0.010}}     % J-K color index from isochrones.
\newcommand{\hatcurISOspecempirical}{K}                            % stellar spectral type
\newcommand{\hatcurISOdRempirical}{\ensuremath{0.0018\pm0.0034}}   % stellar dR from empirical model
\newcommand{\hatcurISOdMbolempirical}{\ensuremath{-0.02\pm0.10}}   % stellar dMbol from empirical model
%% --------------------------------------------------------------------
\newcommand{\hatcurRVKempirical}{\ensuremath{146.4\pm1.1}}         % RV semi-amplitude [m/s]
\newcommand{\hatcurRVrkempirical}{\ensuremath{0\pm0}}              % sqrt(e)*cos(omega)
\newcommand{\hatcurRVrhempirical}{\ensuremath{0\pm0}}              % sqrt(e)*sin(omega)
\newcommand{\hatcurRVkempirical}{\ensuremath{0\pm0}}               % e*cos(omega)
\newcommand{\hatcurRVhempirical}{\ensuremath{0\pm0}}               % e*sin(omega)
\newcommand{\hatcurRVtroneempirical}{\ensuremath{0\pm0}}           % RV linear trend tr1 factor
\newcommand{\hatcurRVtrtwoempirical}{\ensuremath{0\pm0}}           % RV linear trend tr2 factor
\newcommand{\hatcurRVgammaAempirical}{\ensuremath{29.15\pm0.88}}   % RV gamma velocity, relative scale
\newcommand{\hatcurRVjitterAempirical}{\ensuremath{9.6\pm2.6}}     % RV jitter (m/s)
\newcommand{\hatcurRVfitrmsAempirical}{\ensuremath{0.0}}           % RVfitrms
\newcommand{\hatcurRVgammaBempirical}{\ensuremath{-156.4\pm8.7}}   % RV gamma velocity, relative scale
\newcommand{\hatcurRVjitterBempirical}{\ensuremath{5.8\pm2.3}}     % RV jitter (m/s)
\newcommand{\hatcurRVfitrmsBempirical}{\ensuremath{0.0}}           % RVfitrms
\newcommand{\hatcurRVgammaCempirical}{\ensuremath{-8899.4\pm3.3}}  % RV gamma velocity, relative scale
\newcommand{\hatcurRVjitterCempirical}{\ensuremath{20.3\pm7.2}}    % RV jitter (m/s)
\newcommand{\hatcurRVfitrmsCempirical}{\ensuremath{0.0}}           % RVfitrms
\newcommand{\hatcurRVeccenempirical}{\ensuremath{0\pm0}}           % eccentricity
\newcommand{\hatcurRVeccentwosiglimempirical}{\ensuremath{<0.000}} % eccentricity
\newcommand{\hatcurRVomegaempirical}{\ensuremath{0\pm0}}           % argument of pericenter
%% --------------------------------------------------------------------
\newcommand{\hatcurPPiempirical}{\ensuremath{89.26\pm0.18}}        % orbital inclination
\newcommand{\hatcurPPgempirical}{\ensuremath{16.14\pm0.19}}        % planetary surface gravity (m/s^2)
\newcommand{\hatcurPPloggempirical}{\ensuremath{3.2080\pm0.0051}}  % planetary surface gravity (log cgs)
\newcommand{\hatcurPParempirical}{\ensuremath{9.512\pm0.047}}      % relative orbital radius (a/R*)
\newcommand{\hatcurPParelempirical}{\ensuremath{0.03003\pm0.00022}} % semimajor axis (AU)
\newcommand{\hatcurPPrhoempirical}{\ensuremath{0.759\pm0.013}}     % planetary density (cgs)
\newcommand{\hatcurPPmempirical}{\ensuremath{0.738\pm0.012}}       % planetary mass (M_jup)
\newcommand{\hatcurPPmshortempirical}{\ensuremath{0.74}}           % planetary mass (M_jup)
\newcommand{\hatcurPPmlongempirical}{\ensuremath{0.738\pm0.012}}   % planetary mass (M_jup)
\newcommand{\hatcurPPmeempirical}{\ensuremath{234.5\pm3.7}}        % planetary mass (M_earth)
\newcommand{\hatcurPPmeshortempirical}{\ensuremath{234.5}}         % planetary mass (M_earth)
\newcommand{\hatcurPPmelongempirical}{\ensuremath{234.5\pm3.7}}    % planetary mass (M_earth)
\newcommand{\hatcurPPrempirical}{\ensuremath{1.0647\pm0.0091}}     % planetary radius (R_jup)
\newcommand{\hatcurPPrshortempirical}{\ensuremath{1.06}}           % planetary radius (R_jup)
\newcommand{\hatcurPPrlongempirical}{\ensuremath{1.0647\pm0.0091}} % planetary radius (R_jup)
\newcommand{\hatcurPPreempirical}{\ensuremath{11.93\pm0.10}}       % planetary radius (R_earth)
\newcommand{\hatcurPPreshortempirical}{\ensuremath{11.9}}          % planetary radius (R_earth)
\newcommand{\hatcurPPrelongempirical}{\ensuremath{11.93\pm0.10}}   % planetary radius (R_earth)
\newcommand{\hatcurPPmrcorrempirical}{\ensuremath{0.76}}           % mass/radius correlation
\newcommand{\hatcurPPteffempirical}{\ensuremath{966.3\pm8.4}}      % planetary temperature (K)
\newcommand{\hatcurPPthetaempirical}{\ensuremath{0.06080\pm0.00061}} % Safranov number
\newcommand{\hatcurPPfluxperiempirical}{\ensuremath{1.972\pm0.069}} % flux @ periastron (CGS)
\newcommand{\hatcurPPfluxperidimempirical}{\ensuremath{8}}         % flux @ periastron (CGS) units.
\newcommand{\hatcurPPfluxapempirical}{\ensuremath{1.972\pm0.069}}  % flux @ apastron (CGS)
\newcommand{\hatcurPPfluxapdimempirical}{\ensuremath{8}}           % flux @ apastron (CGS) units.
\newcommand{\hatcurPPfluxavgempirical}{\ensuremath{1.972\pm0.069}} % flux on average (CGS)
\newcommand{\hatcurPPfluxavgdimempirical}{\ensuremath{8}}          % flux average (CGS) units.
\newcommand{\hatcurPPfluxavglogempirical}{\ensuremath{8.295\pm0.015}} % log10 flux on average (CGS)
%% --------------------------------------------------------------------
\newcommand{\hatcurXsecphaseempirical}{\ensuremath{0\pm0}}         % Phase of secondary eclipse
\newcommand{\hatcurXsecondaryempirical}{\ensuremath{2456921.041180\pm0.000062}} % Secondary eclipse epoch
\newcommand{\hatcurXsecdurempirical}{\ensuremath{0.08700\pm0.00031}} % sec eclipse duration (days)
\newcommand{\hatcurXsecingdurempirical}{\ensuremath{0.012233\pm0.000095}} % sec I/E duration (days)
\newcommand{\hatcurPPphiconjempirical}{\ensuremath{0\pm0}}         % phase diff between conjunction and periastron
\newcommand{\hatcurPPperiempirical}{\ensuremath{2456919.317374\pm0.000062}} % time of periastron passage.
\newcommand{\hatcurPPaequivempirical}{\ensuremath{0.0832\pm0.0015}} % equivalent semi-major axis
\newcommand{\hatcurPPtcircempirical}{\ensuremath{47.0\pm1.3}}      % circularization timescale
\newcommand{\hatcurPPtinfallempirical}{\ensuremath{1579\pm45}}     % infall timescale
%% --------------------------------------------------------------------
\newcommand{\hatcurXdistempirical}{\ensuremath{184.1\pm3.0}}       % distance (pc), no reddenning correction
\newcommand{\hatcurXAvempirical}{\ensuremath{0.117\pm0.050}}       % Av (mag)
\newcommand{\hatcurXdistredempirical}{\ensuremath{184.1\pm3.0}}    % distance with Av correction (pc)
\newcommand{\hatcurXEBVempirical}{\ensuremath{0.038\pm0.016}}      % E(B-V) (mag)
\newcommand{\hatcurXmvisoredempirical}{\ensuremath{13.816\pm0.061}} % Expected m_v with reddening (mag)
\newcommand{\hatcurXmiisoredempirical}{\ensuremath{100\pm0}}       % Expected m_i with reddening (mag)
\newcommand{\hatcurXmjisoredempirical}{\ensuremath{11.941\pm0.018}} % Expected m_j with reddening (mag)
\newcommand{\hatcurXmhisoredempirical}{\ensuremath{11.165\pm0.015}} % Expected m_h with reddening (mag)
\newcommand{\hatcurXmkisoredempirical}{\ensuremath{11.027\pm0.015}} % Expected m_k with reddening (mag)
\newcommand{\hatcurXviisoredempirical}{\ensuremath{100\pm0}}       % Expected V-I with reddening (mag)
\newcommand{\hatcurXvkisoredempirical}{\ensuremath{2.789\pm0.063}} % Expected V-K with reddening (mag)
\newcommand{\hatcurXjhisoredempirical}{\ensuremath{0.777_{-0.017}^{+0.013}}} % Expected J-H with reddening (mag)
\newcommand{\hatcurXjkisoredempirical}{\ensuremath{0.915_{-0.015}^{+0.011}}} % Expected J-K with reddening (mag)
\newcommand{\hatcurCCpmraempirical}{\ensuremath{-19.5\pm2.5}}      % proper motion, in RA
\newcommand{\hatcurCCpmdecempirical}{\ensuremath{-3.2\pm2.8}}      % proper motion, in DEC
\newcommand{\hatcurCCpmempirical}{\ensuremath{19.8\pm3.8}}         % proper motion


==> HTR268-002.tex <==
\newcommand{\hatcurhtr}{HTR268-002}                       % Original HTR name of target
\newcommand{\hatcurfield}{\ensuremath{string}}            % HTR field
\newcommand{\hatcurCCra}{\ensuremath{07^{\mathrm h}53^{\mathrm m}55.97{\mathrm s}}}                     % Right Ascension
\newcommand{\hatcurCCdec}{\ensuremath{+23{\arcdeg}56{\arcmin}17.6{\arcsec}}}                    % Declination
\newcommand{\hatcurCCmag}{14.020}                         % apparent V-band magnitude
\newcommand{\hatcurCCtwomass}{2MASS~07535598+2356176}     % 2MASS identifier
\newcommand{\hatcurCCgsc}{GSC~1925-01046}                 % GSC(1.2) identifier
\newcommand{\hatcurCCtassmv}{\ensuremath{14.020\pm0.079}} % APASS V-band magnitude
\newcommand{\hatcurCCtassmvshort}{\ensuremath{14.0}}      % APASS V-band magnitude
\newcommand{\hatcurCCtassmB}{\ensuremath{15.32\pm0.17}}   % APASS B-band magnitude
\newcommand{\hatcurCCtassmBshort}{\ensuremath{15.3}}      % APASS B-band magnitude
\newcommand{\hatcurCCtassmI}{\ensuremath{nff\pmnff}}      % TASS I-band magnitude
\newcommand{\hatcurCCtassmIshort}{\ensuremath{0.0}}       % TASS I-band magnitude
\newcommand{\hatcurCCtassmg}{\ensuremath{14.71\pm0.13}}   % APASS g-band magnitude
\newcommand{\hatcurCCtassmgshort}{\ensuremath{14.7}}      % APASS g-band magnitude
\newcommand{\hatcurCCtassmr}{\ensuremath{13.485\pm0.076}} % APASS r-band magnitude
\newcommand{\hatcurCCtassmrshort}{\ensuremath{13.5}}      % APASS r-band magnitude
\newcommand{\hatcurCCtassmi}{\ensuremath{13.25\pm0.42}}   % APASS i-band magnitude
\newcommand{\hatcurCCtassmishort}{\ensuremath{13.2}}      % APASS i-band magnitude
%% --------------------------------------------------------------------
\newcommand{\hatcurCCtwomassJmag}{\ensuremath{11.750\pm0.022}} % 2MASS ORIG MAG
\newcommand{\hatcurCCtwomassHmag}{\ensuremath{11.210\pm0.023}} % 2MASS ORIG MAG
\newcommand{\hatcurCCtwomassKmag}{\ensuremath{11.019\pm0.018}} % 2MASS ORIG MAG
\newcommand{\hatcurCCcitJmag}{\ensuremath{11.748\pm0.023}} % 2MASS CIT MAG
\newcommand{\hatcurCCcitHmag}{\ensuremath{11.202\pm0.024}} % 2MASS CIT MAG
\newcommand{\hatcurCCcitKmag}{\ensuremath{11.043\pm0.019}} % 2MASS CIT MAG
\newcommand{\hatcurCCbbJmag}{\ensuremath{11.826\pm0.025}} % 2MASS BB MAG
\newcommand{\hatcurCCbbHmag}{\ensuremath{11.226\pm0.025}} % 2MASS BB MAG
\newcommand{\hatcurCCbbKmag}{\ensuremath{11.063\pm0.019}} % 2MASS BB MAG
\newcommand{\hatcurCCesoJmag}{\ensuremath{11.833\pm0.029}} % 2MASS ESO MAG
\newcommand{\hatcurCCesoHmag}{\ensuremath{11.225\pm0.036}} % 2MASS ESO MAG
\newcommand{\hatcurCCesoKmag}{\ensuremath{11.060\pm0.020}} % 2MASS ESO MAG
\newcommand{\hatcurCCesoJHmag}{\ensuremath{0.608\pm0.043}} % 2MASS ESO JH COLOR
\newcommand{\hatcurCCesoJKmag}{\ensuremath{0.773\pm0.033}} % 2MASS ESO JK COLOR
\newcommand{\hatcurCCesoHKmag}{\ensuremath{0.165\pm0.040}} % 2MASS ESO HK COLOR
%% --------------------------------------------------------------------
\newcommand{\hatcurLCdip}{\ensuremath{3.6}}               % BLS detected dip (mmag)
\newcommand{\hatcurLCrprstar}{\ensuremath{0.1633\pm0.0011}} % Rp/R*
\newcommand{\hatcurLCbsq}{\ensuremath{0.043_{-0.024}^{+0.033}}} % impact parameter square
\newcommand{\hatcurLCimp}{\ensuremath{0.206_{-0.070}^{+0.069}}} % impact parameter
\newcommand{\hatcurLCzeta}{\ensuremath{26.795_{-0.069}^{+0.106}}} % zeta/R*
\newcommand{\hatcurLCdur}{\ensuremath{0.08743\pm0.00048}} % transit duration (days)
\newcommand{\hatcurLCdurshort}{\ensuremath{0.0874}}       % transit duration (days)
\newcommand{\hatcurLCdurhr}{\ensuremath{2.098\pm0.012}}   % transit duration (hours)
\newcommand{\hatcurLCdurhrshort}{\ensuremath{2.098}}      % transit duration (hours)
\newcommand{\hatcurLCq}{\ensuremath{0.03800\pm0.00021}}   % fractional transit duration (days)
\newcommand{\hatcurLCqshort}{\ensuremath{0.038}}          % fractional transit duration (days)
\newcommand{\hatcurLCingdur}{\ensuremath{0.01275\pm0.00037}} % ingress/egress duration (days)
\newcommand{\hatcurLCP}{\ensuremath{2.29840546\pm0.00000052}} % period (days)
\newcommand{\hatcurLCPprec}{\ensuremath{2.2984055}}       % period (days)
\newcommand{\hatcurLCPshort}{\ensuremath{2.2984}}         % period (days)
\newcommand{\hatcurLCT}{\ensuremath{2456949.77075\pm0.00012}} % epoch (BJD)
\newcommand{\hatcurLCTA}{\ensuremath{2455876.41534\pm0.00028}} % TA (BJD)
\newcommand{\hatcurLCTB}{\ensuremath{2457480.70237\pm0.00016}} % TB (BJD)
\newcommand{\hatcurLChatnetm}{\ensuremath{13.44089\pm0.00023}} % HATNet OOT level
\newcommand{\hatcurLCiblend}{\ensuremath{0.876\pm0.037}}  % HATNet iblend factor
\newcommand{\hatcurLCrho}{\ensuremath{2.49_{-1.08}^{+0.82}}} % stellar density no isochrone constraint (cgs)
%% --------------------------------------------------------------------
\newcommand{\hatcurSMEiteff}{\ensuremath{4514\pm50}}      % Ini SME, stellar effective temperature
\newcommand{\hatcurSMEizfeh}{\ensuremath{-0.140\pm0.080}} % Ini SME, stellar metallicity
\newcommand{\hatcurSMEizfehshort}{\ensuremath{-0.14}}     % Ini SME, stellar metallicity
\newcommand{\hatcurSMEilogg}{\ensuremath{4.67\pm0.10}}    % Ini SME, stellar surface gravity
\newcommand{\hatcurSMEivsin}{\ensuremath{0.0\pm2.0}}      % Ini SME, stellar rotational velocity
\newcommand{\hatcurSMEivmac}{\ensuremath{nff\pmnff}}      % Ini SME, stellar macroturbulence
\newcommand{\hatcurSMEivmic}{\ensuremath{nff\pmnff}}      % Ini SME, stellar microturbulence
%% --------------------------------------------------------------------
\newcommand{\hatcurLBiz}{\ensuremath{0.3598}}             % Limb darkening parameters, Gamma1, z-band
\newcommand{\hatcurLBiiz}{\ensuremath{0.2452}}            % Limb darkening parameters, Gamma2, z-band
\newcommand{\hatcurLBii}{\ensuremath{0.4552}}             % Limb darkening parameters, Gamma1, i-band
\newcommand{\hatcurLBiii}{\ensuremath{0.2183}}            % Limb darkening parameters, Gamma2, i-band
\newcommand{\hatcurLBiI}{\ensuremath{0.4216}}             % Limb darkening parameters, Gamma1, I-band
\newcommand{\hatcurLBiiI}{\ensuremath{0.2285}}            % Limb darkening parameters, Gamma2, I-band
\newcommand{\hatcurLBig}{\ensuremath{0.8947}}             % Limb darkening parameters, Gamma1, g-band
\newcommand{\hatcurLBiig}{\ensuremath{-0.0532}}           % Limb darkening parameters, Gamma2, g-band
\newcommand{\hatcurLBir}{\ensuremath{0.6186}}             % Limb darkening parameters, Gamma1, r-band
\newcommand{\hatcurLBiir}{\ensuremath{0.1455}}            % Limb darkening parameters, Gamma2, r-band
\newcommand{\hatcurLBiR}{\ensuremath{0.5726}}             % Limb darkening parameters, Gamma1, R-band
\newcommand{\hatcurLBiiR}{\ensuremath{0.1672}}            % Limb darkening parameters, Gamma2, R-band
\newcommand{\hatcurLBikep}{\ensuremath{0.1000}}           % Limb darkening parameters, Gamma1, Kep-band
\newcommand{\hatcurLBiikep}{\ensuremath{0.1000}}          % Limb darkening parameters, Gamma2, Kep-band
%% --------------------------------------------------------------------
\newcommand{\hatcurISOm}{\ensuremath{0.671\pm0.021}}      % stellar mass
\newcommand{\hatcurISOmshort}{\ensuremath{0.67}}          % stellar mass
\newcommand{\hatcurISOmlong}{\ensuremath{0.671\pm0.021}}  % stellar mass
\newcommand{\hatcurISOr}{\ensuremath{0.611_{-0.021}^{+0.029}}} % stellar radius
\newcommand{\hatcurISOrshort}{\ensuremath{0.61}}          % stellar radius
\newcommand{\hatcurISOrlong}{\ensuremath{0.611_{-0.021}^{+0.029}}} % stellar radius
\newcommand{\hatcurISOrho}{\ensuremath{4.15\pm0.40}}      % stellar density (cgs)
\newcommand{\hatcurISOrholong}{\ensuremath{4.15\pm0.40}}  % stellar density (cgs)
\newcommand{\hatcurISOlogg}{\ensuremath{4.691\pm0.026}}   % stellar surface gravity from isochrones
\newcommand{\hatcurISOlum}{\ensuremath{0.141\pm0.016}}    % stellar luminosity
\newcommand{\hatcurISOlumshort}{\ensuremath{0.14}}        % stellar luminosity
\newcommand{\hatcurISOmv}{\ensuremath{7.40\pm0.15}}       % stellar absolute magnitude
\newcommand{\hatcurISOvi}{\ensuremath{1.161\pm0.041}}     % stellar V-I index
\newcommand{\hatcurISOage}{\ensuremath{7.6_{-7.0}^{+4.2}}} % stellar age
\newcommand{\hatcurISOsigma}{\ensuremath{0.00190\pm0.00043}} % system mass-correction sigma parameter
\newcommand{\hatcurISOMJ}{\ensuremath{5.42\pm0.11}}       % stellar absolute J magnitude
\newcommand{\hatcurISOMH}{\ensuremath{4.83\pm0.11}}       % stellar absolute H magnitude
\newcommand{\hatcurISOMK}{\ensuremath{4.73\pm0.11}}       % stellar absolute K magnitude
\newcommand{\hatcurISOJK}{\ensuremath{0.690\pm0.020}}     % J-K color index from isochrones.
\newcommand{\hatcurISOspec}{K}                            % stellar spectral type
%% --------------------------------------------------------------------
\newcommand{\hatcurRVK}{\ensuremath{142.1\pm8.4}}         % RV semi-amplitude [m/s]
\newcommand{\hatcurRVrk}{\ensuremath{0.016_{-0.078}^{+0.034}}} % sqrt(e)*cos(omega)
\newcommand{\hatcurRVrh}{\ensuremath{-0.293_{-0.046}^{+0.063}}} % sqrt(e)*sin(omega)
\newcommand{\hatcurRVk}{\ensuremath{0.005_{-0.024}^{+0.013}}} % e*cos(omega)
\newcommand{\hatcurRVh}{\ensuremath{-0.087\pm0.031}}      % e*sin(omega)
\newcommand{\hatcurRVtrone}{\ensuremath{0\pm0}}           % RV linear trend tr1 factor
\newcommand{\hatcurRVtrtwo}{\ensuremath{0\pm0}}           % RV linear trend tr2 factor
\newcommand{\hatcurRVgammaA}{\ensuremath{39.3\pm7.1}}     % RV gamma velocity, relative scale
\newcommand{\hatcurRVjitterA}{\ensuremath{16.7\pm5.5}}    % RV jitter (m/s)
\newcommand{\hatcurRVjittertwosiglimA}{\ensuremath{<29.4}} % RV jitter (m/s) 95 percent confidence upper limit
\newcommand{\hatcurRVfitrmsA}{\ensuremath{0.0}}           % RVfitrms
\newcommand{\hatcurRVgammaB}{\ensuremath{-153\pm30}}      % RV gamma velocity, relative scale
\newcommand{\hatcurRVjitterB}{\ensuremath{0\pm19}}        % RV jitter (m/s)
\newcommand{\hatcurRVjittertwosiglimB}{\ensuremath{<17.7}} % RV jitter (m/s) 95 percent confidence upper limit
\newcommand{\hatcurRVfitrmsB}{\ensuremath{0.0}}           % RVfitrms
\newcommand{\hatcurRVgammaC}{\ensuremath{-8883\pm20}}     % RV gamma velocity, relative scale
\newcommand{\hatcurRVjitterC}{\ensuremath{0\pm14}}        % RV jitter (m/s)
\newcommand{\hatcurRVjittertwosiglimC}{\ensuremath{<35.6}} % RV jitter (m/s) 95 percent confidence upper limit
\newcommand{\hatcurRVfitrmsC}{\ensuremath{0.0}}           % RVfitrms
\newcommand{\hatcurRVeccen}{\ensuremath{0.092\pm0.032}}   % eccentricity
\newcommand{\hatcurRVeccentwosiglim}{\ensuremath{<0.150}} % eccentricity
\newcommand{\hatcurRVomega}{\ensuremath{273\pm18}}        % argument of pericenter
%% --------------------------------------------------------------------
\newcommand{\hatcurPPi}{\ensuremath{88.98\pm0.30}}        % orbital inclination
\newcommand{\hatcurPPg}{\ensuremath{18.1\pm1.7}}          % planetary surface gravity (m/s^2)
\newcommand{\hatcurPPlogg}{\ensuremath{3.258\pm0.039}}    % planetary surface gravity (log cgs)
\newcommand{\hatcurPPar}{\ensuremath{10.50_{-0.41}^{+0.32}}} % relative orbital radius (a/R*)
\newcommand{\hatcurPParel}{\ensuremath{0.02984\pm0.00031}} % semimajor axis (AU)
\newcommand{\hatcurPPrho}{\ensuremath{0.94\pm0.12}}       % planetary density (cgs)
\newcommand{\hatcurPPm}{\ensuremath{0.705_{-0.054}^{+0.033}}} % planetary mass (M_jup)
\newcommand{\hatcurPPmshort}{\ensuremath{0.70}}           % planetary mass (M_jup)
\newcommand{\hatcurPPmlong}{\ensuremath{0.705_{-0.054}^{+0.033}}} % planetary mass (M_jup)
\newcommand{\hatcurPPme}{\ensuremath{224_{-17}^{+10}}}    % planetary mass (M_earth)
\newcommand{\hatcurPPmeshort}{\ensuremath{224.0}}         % planetary mass (M_earth)
\newcommand{\hatcurPPmelong}{\ensuremath{224_{-17}^{+10}}} % planetary mass (M_earth)
\newcommand{\hatcurPPr}{\ensuremath{0.974\pm0.038}}       % planetary radius (R_jup)
\newcommand{\hatcurPPrshort}{\ensuremath{0.97}}           % planetary radius (R_jup)
\newcommand{\hatcurPPrlong}{\ensuremath{0.974\pm0.038}}   % planetary radius (R_jup)
\newcommand{\hatcurPPre}{\ensuremath{10.91\pm0.43}}       % planetary radius (R_earth)
\newcommand{\hatcurPPreshort}{\ensuremath{10.9}}          % planetary radius (R_earth)
\newcommand{\hatcurPPrelong}{\ensuremath{10.91\pm0.43}}   % planetary radius (R_earth)
\newcommand{\hatcurPPmrcorr}{\ensuremath{0.17}}           % mass/radius correlation
\newcommand{\hatcurPPteff}{\ensuremath{991\pm23}}         % planetary temperature (K)
\newcommand{\hatcurPPtheta}{\ensuremath{0.0636\pm0.0046}} % Safranov number
\newcommand{\hatcurPPfluxperi}{\ensuremath{2.63\pm0.15}}  % flux @ periastron (CGS)
\newcommand{\hatcurPPfluxperidim}{\ensuremath{8}}         % flux @ periastron (CGS) units.
\newcommand{\hatcurPPfluxap}{\ensuremath{1.81_{-0.23}^{+0.34}}} % flux @ apastron (CGS)
\newcommand{\hatcurPPfluxapdim}{\ensuremath{8}}           % flux @ apastron (CGS) units.
\newcommand{\hatcurPPfluxavg}{\ensuremath{2.18_{-0.19}^{+0.25}}} % flux on average (CGS)
\newcommand{\hatcurPPfluxavgdim}{\ensuremath{8}}          % flux average (CGS) units.
\newcommand{\hatcurPPfluxavglog}{\ensuremath{8.338\pm0.041}} % log10 flux on average (CGS)
%% --------------------------------------------------------------------
\newcommand{\hatcurXsecphase}{\ensuremath{0.503\pm0.016}} % Phase of secondary eclipse
\newcommand{\hatcurXsecondary}{\ensuremath{2456950.927\pm0.037}} % Secondary eclipse epoch
\newcommand{\hatcurXsecdur}{\ensuremath{0.0733\pm0.0045}} % sec eclipse duration (days)
\newcommand{\hatcurXsecingdur}{\ensuremath{0.01054\pm0.00070}} % sec I/E duration (days)
\newcommand{\hatcurPPphiconj}{\ensuremath{0.469_{-0.940}^{+0.019}}} % phase diff between conjunction and periastron
\newcommand{\hatcurPPperi}{\ensuremath{2456948.7\pm1.3}}  % time of periastron passage.
\newcommand{\hatcurPPaequiv}{\ensuremath{0.0794\pm0.0038}} % equivalent semi-major axis
\newcommand{\hatcurPPtcirc}{\ensuremath{65.3\pm9.8}}      % circularization timescale
\newcommand{\hatcurPPtinfall}{\ensuremath{2640\pm450}}    % infall timescale
%% --------------------------------------------------------------------
\newcommand{\hatcurXdist}{\ensuremath{185.0\pm9.2}}       % distance (pc), no reddenning correction
\newcommand{\hatcurXAv}{\ensuremath{0.34\pm0.11}}         % Av (mag)
\newcommand{\hatcurXdistred}{\ensuremath{182.7\pm8.8}}    % distance with Av correction (pc)
\newcommand{\hatcurXEBV}{\ensuremath{0.111\pm0.035}}      % E(B-V) (mag)
\newcommand{\hatcurXmvisored}{\ensuremath{14.051\pm0.072}} % Expected m_v with reddening (mag)
\newcommand{\hatcurXmiisored}{\ensuremath{12.711\pm0.030}} % Expected m_i with reddening (mag)
\newcommand{\hatcurXmjisored}{\ensuremath{11.818\pm0.016}} % Expected m_j with reddening (mag)
\newcommand{\hatcurXmhisored}{\ensuremath{11.200\pm0.015}} % Expected m_h with reddening (mag)
\newcommand{\hatcurXmkisored}{\ensuremath{11.073\pm0.017}} % Expected m_k with reddening (mag)
\newcommand{\hatcurXviisored}{\ensuremath{1.339\pm0.047}} % Expected V-I with reddening (mag)
\newcommand{\hatcurXvkisored}{\ensuremath{2.978\pm0.078}} % Expected V-K with reddening (mag)
\newcommand{\hatcurXjhisored}{\ensuremath{0.6180\pm0.0089}} % Expected J-H with reddening (mag)
\newcommand{\hatcurXjkisored}{\ensuremath{0.746\pm0.015}} % Expected J-K with reddening (mag)
\newcommand{\hatcurCCpmra}{\ensuremath{-19.5\pm2.5}}      % proper motion, in RA
\newcommand{\hatcurCCpmdec}{\ensuremath{-3.2\pm2.8}}      % proper motion, in DEC
\newcommand{\hatcurCCpm}{\ensuremath{19.8\pm3.8}}         % proper motion


==> newcommand_spec_multi_template.tex <==
%% GB's various newcommands for making editing easy for this specific paper

% This is the template version to be used for planets announced in a
% multi-planet paper. This file should be filled in separately for
% each planet in the paper. You should also find/replace the term
% xxxxx below with a unique identifier for each planet (e.g. xxxxA for
% the first one).  A version of this file should be saved with a
% unique name in the document directory for each planet, and all files
% should be processed into the newcommand_spec_multi.tex file using
% the scr/makenewcommand_spec_multi.sh script. This is done to allow
% you to reference planet information using commands like \hatcur{14}
% rather than \hatcurxxxxA. The newcommand_spec_multi.tex file so
% generated should not need to be edited or regenerated if changes are
% made to any of the planets parameters. Any changes should be made to
% the planet's own newcommand_spec.tex file.

% -------- Aliases specific to this paper/planet which should be edited -------

% The name of the host star and/or the planet:
\newcommand{\hatcurxxxxx}{HAT-P-14}
\newcommand{\hatcurbxxxxx}{HAT-P-14b}
\newcommand{\hatcurcxxxxx}{HAT-P-14c}

% The number used to index this system in the paper
\newcommand{\hatcurplanetnumxxxxx}{14}

%\newcommand{\hatcurCCraxxxxx}{\ensuremath{08^{\mathrm h}39^{\mathrm m}31.82^{\mathrm s}}}  % right ascension
%\newcommand{\hatcurCCdecxxxxx}{\ensuremath{+47^{\mathrm d}21^{\mathrm m}07.4^{\mathrm s}}} % declination

\newcommand{\hatcurRVgammaabsxxxxx}{\hatcurDSgamma{\hatcurplanetnumxxxxx}}                           % Absolute Gamma velocity

\newcommand{\hatcurRVgammarelxxxxx}{\hatcurRVgamma{\hatcurplanetnumxxxxx}}                           % Relative Gamma velocity. Typically that of the Keck RVs.

\newcommand{\hatcurCCtassvixxxxx}{\ensuremath{0.527\pm0.12}}                  % TASS V-I

\newcommand{\hatcurSMEversionxxxxx}{ii}                                       % Final SME version:i or ii?

% Isochrones used for this planet.
\newcommand{\hatcurisoshortxxxxx}{YY}
%\newcommand{\hatcurisoshortxxxxx}{Baraffe}
\newcommand{\hatcurisofullxxxxx}{Yonsei-Yale (YY)}
%\newcommand{\hatcurisofullxxxxx}{Baraffe}
\newcommand{\hatcurisocitexxxxx}{yi:2001}
%\newcommand{\hatcurisocitexxxxx}{baraffe:1998}

% Luminosity indicator used for this planet.
\newcommand{\hatcurlumindxxxxx}{\arstar}
%\newcommand{\hatcurlumindxxxxx}{Hip}s

% JHK filter type for the isochrone set used for this planet.
\newcommand{\hatcurjhkfilsetxxxxx}{ESO}
%\newcommand{\hatcurjhkfilsetxxxxx}{BB}
%\newcommand{\hatcurjhkfilsetxxxxx}{CIT}

% --------------------------------------------------------------------------
% The aliases below should not need editing, other than replaceing xxxxxx
% to whatever string.
% 
\newcommand{\hatcurSMEteffxxxxx}{\ifthenelse{\equal{\hatcurSMEversionxxxxx}{i}}{\hatcurSMEiteff{\hatcurplanetnumxxxxx}}{\hatcurSMEiiteff{\hatcurplanetnumxxxxx}}}
\newcommand{\hatcurSMEzfehxxxxx}{\ifthenelse{\equal{\hatcurSMEversionxxxxx}{i}}{\hatcurSMEizfeh{\hatcurplanetnumxxxxx}}{\hatcurSMEiizfeh{\hatcurplanetnumxxxxx}}}
\newcommand{\hatcurSMEzfehshortxxxxx}{\ifthenelse{\equal{\hatcurSMEversionxxxxx}{i}}{\hatcurSMEizfehshort{\hatcurplanetnumxxxxx}}{\hatcurSMEiizfehshort{\hatcurplanetnumxxxxx}}}
\newcommand{\hatcurSMEloggxxxxx}{\ifthenelse{\equal{\hatcurSMEversionxxxxx}{i}}{\hatcurSMEilogg{\hatcurplanetnumxxxxx}}{\hatcurSMEiilogg{\hatcurplanetnumxxxxx}}}
\newcommand{\hatcurSMEvsinxxxxx}{\ifthenelse{\equal{\hatcurSMEversionxxxxx}{i}}{\hatcurSMEivsin{\hatcurplanetnumxxxxx}}{\hatcurSMEiivsin{\hatcurplanetnumxxxxx}}}
\newcommand{\hatcurSMEvmacxxxxx}{\ifthenelse{\equal{\hatcurSMEversionxxxxx}{i}}{\hatcurSMEivmac{\hatcurplanetnumxxxxx}}{\hatcurSMEiivmac{\hatcurplanetnumxxxxx}}}
\newcommand{\hatcurSMEvmicxxxxx}{\ifthenelse{\equal{\hatcurSMEversionxxxxx}{i}}{\hatcurSMEivmic{\hatcurplanetnumxxxxx}}{\hatcurSMEiivmic{\hatcurplanetnumxxxxx}}}

